Open-world Text-specified Object Counting

Our objective is open-world object counting in images, where the target object class is specified by a text description. To this end, we propose CounTX, a class-agnostic, single-stage model using a transformer decoder counting head on top of pre-trained joint text-image representations. CounTX is able to count the number of instances of any class given only an image and a text description of the target object class, and can be trained end-to-end. In addition to this model, we make the following contributions: (i) we compare the performance of CounTX to prior work on open-world object counting, and show that our approach exceeds the state of the art on all measures on the FSC-147 benchmark for methods that use text to specify the task; (ii) we present and release FSC-147-D, an enhanced version of FSC-147 with text descriptions, so that object classes can be described with more detailed language than their simple class names. FSC-147-D and the code are available at https://www.robots.ox.ac.uk/~vgg/research/countx.

==> sections/abstract.tex <==
\begin{abstract}
Our objective is open-world object counting in images, where the target object class is specified by a text description. To this end, we propose {\em CounTX}, a class-agnostic, single-stage model using a transformer decoder counting head on top of pre-trained joint text-image representations. CounTX is able to count the number of instances of any class given only an image and a text description of the target object class, and can be trained end-to-end. 
%To the best of our knowledge, we are the first to tackle the open-world counting problem in this way. 
In addition to this model, we make the following contributions: (i) we compare the performance of CounTX to prior work on open-world object counting, and show that our approach exceeds the state of the art on all measures on the FSC-147~\cite{m_Ranjan-etal-CVPR21} benchmark for methods that use text to specify the task; (ii) we present and release FSC-147-D, an enhanced version of FSC-147 with text descriptions, so that object classes can be described with more detailed language than their simple class names. FSC-147-D and the code are available at \href{https://www.robots.ox.ac.uk/~vgg/research/countx}{https://www.robots.ox.ac.uk/\textasciitilde vgg/research/countx}.

% Our objective is open-world object counting in images, where the target object class is specified by a text description. To this end, we propose a class agnostic single-stage model using a transformer encoder counting head on top of a pre-trained joint text-image representations. The model is able to count the number of instances of any class given only an image and a text description of the target object class, and can be trained end-to-end. To the best of our knowledge, we are the first to tackle the open-world counting problem in this way. Apart from the model, we make the following contributions: (i) we compare the performance of the model to prior work on open-world object counting, and show that our approach exceeds the state of the art on all measures on the FSC-147~\cite{m_Ranjan-etal-CVPR21} benchmark for methods that use text or a class name to specify the task; (ii) we provide and will release text descriptions for the classes in the FSC-147 dataset, so that object classes can be described in more detail than simply the class name.

%Specifically, our model is composed of pretrained image
% and text encoders that map the image and class description to a
% fine-tuned image-text embedding space. The image and text embeddings
% from these encoders are passed through transformer decoder layers that
% output spatial feature maps used to regress the object count. We
% verify the effectiveness of our approach on an extended version of the
% FSC-147 dataset through both quantitative and qualitative results. Our
% method significantly improves on both the validation set and test set
% errors presented in the only prior work on zero-shot object
% counting.
\end{abstract}
